On the Domain Generalizability of RF Fingerprints Through Multifractal Dimension Representation

RF data-driven device fingerprinting through the use of deep learning has recently surfaced as a possible method for enabling secure device identification and authentication. Traditional approaches are commonly susceptible to the domain adaptation problem where a model trained on data collected under one domain performs badly when tested on data collected under a different domain. Some examples of a domain change include varying the location or environment of the device and varying the time or day of the data collection. In this work, we propose using multifractal analysis and the variance fractal dimension trajectory (VFDT) as a data representation input to the deep neural network to extract device fingerprints that are domain generalizable. We analyze the effectiveness of the proposed VFDT representation in detecting device-specific signatures from hardware-impaired IQ (in-phase and quadrature) signals, and we evaluate its robustness in real-world settings, using an experimental testbed of 30 WiFi-enabled Pycom devices. Our experimental results show that the proposed VFDT representation improves the scalability, robustness and generalizability of the deep learning models significantly compared to when using IQ data samples.

==> Comments.tex <==
%%% 6/8/22
- add a couple of sentences at the begining of each section (e.g., Sec V.) introducuing the scope of the section

section: experimental setup
- [DONE] DNN section needs to be moved to Results section
- [DONE] exprimental scenarios: put in a table could be better; there is some redundacy with Same Tx, Different Tx etc.

section: results:
- [DONE] did you define what 'vanilla' model is?
- [DONE] caption of subfigure should be done via caption, not adding (a) etc. Did fig 13

NOTES:

I have modified the `closed-set' evaluation sections (hardware, channel, and configuration portability). >>>Let me know if these parts need further work.<<<

I have removed the background section in favor of integrating the background into the 'proposed technique' section. 

I also removed the background information on the hardware impairments...this is because they have been well covered in other works on RF fingerprinting, and my work does not rely on the particular extraction of one kind of impairment (was excessive background for my technique)


I still need to:
- Edit the `open-set' evaluation section (I plan on making this similar to the current `closed-set' section)
- Edit the first few paragraphs of the 'proposedtechnique.tex' section (needs to reflect changes in this section)


==> related.tex <==


%main structure for section

%some look at preprocessing

%some look calibrating model itself

%some look at only scalability and real world 

%some look at deep fingerprint analysis but then no domain (other fractal dimension paper)

%

Existing works attempting to overcome the domain adaptation problem focus on a variety of methods. Some look at using a certain type of preprocessing to extract a single, specific hardware feature, such as the CFO, for example \cite{joo2020hold}. Others use various custom types of preprocessing to help extract an overall fingerprint, independent of domain, that is then passed through a deep learning model for classification \cite{9732439}, \cite{shen2021scalable}. There are also attempts to directly calibrate the model itself to overcome portability problems across domains \cite{gaskin2022tweak}. 

Aside from focusing on domain adaptation, related works also approach other issues with device fingerprinting including scalability \cite{9771750} and signal interference \cite{10.1145/3522783.3529520}. Alternatively, \cite{10012578} proposes using a more complex device fingerprint by combining several different features, including the fractal dimension which is a component of multifractal analysis, for use in a deep learning model. While they consider basic channel noise, complex domain adaptation is not explored. This work looks at analysis of the fundamental device fingerprint with multifractal analysis while also exploring its robustness across domains and scale. 

==> vfdt.tex <==
In this paper, the main method of multifractal analysis used involves estimating the variance fractal dimension of the RF signals. The variance fractal dimension is based on analyzing the statistical variance of the signal amplitude over different scales and ranges. In order to estimate the variance fractal dimension of a signal, it is first assumed that the signal, over a time interval \(\triangle t = t_2 - t_1\), adheres to the following power law relationship

\begin{equation}
    var[x(t_2)-x(t_1)] \sim |t_2-t_1|^{2H}
\end{equation}

where \(x(t)\) is the signal and \(H\) is the Hurst exponent \cite{1532616}. From this assumed power law relationship, the Hurst exponent can be solved for by taking the log of both sides and found to be

\begin{equation}
    H = \lim_{\triangle t \to 0} \frac{1}{2} \frac{\log[var(\triangle x)_{\triangle t}]}{\log(\triangle t)}
\end{equation}

From here, the variance fractal dimension, \(D\), is then related to the Hurst exponent by

\begin{equation}
    D = E + 1 - H \label{eq:fractal dimension}
\end{equation}

where \(E\) is the Euclidean dimension \cite{1225951}. Since all of the base RF signals are 1-dimensional, after the in-phase and quadrature components are separated, \(E\) is set to 1. This simplifies \eqref{eq:fractal dimension} to 

\begin{equation}
    D = 2 - H   \label{eq:final dim}
\end{equation}

In \eqref{eq:final dim}, \(D\) represents the fractal dimension of the overall signal but for the RF signals analyzed in this paper it is more useful to see how the fractal dimension of the signal changes over time. As such a rolling trajectory of the fractal dimension can be taken. This rolling trajectory is called the Variance Fractal Dimension Trajectory (VFDT).

To actually calculate the VFDT of a discrete-time signal, the fractal dimension, \(D\), is calculated for a windowed segment of the base signal. This windowed segment is then shifted or offset by a fixed, predetermined amount of samples and then the fractal dimension of this new segment is taken. The process is then repeated until the end of the signal is reached. Due to the signal being discrete, the length of the windowed segment, \(\triangle w\), is used as the time interval \(\triangle t\). As a result the VFDT, \(D(i)\), of a given windowed segment, \(i\), is

\begin{equation}
    D(i) = 2 - \frac{1}{2} \frac{\log[var(\triangle x)_{\triangle w}]}{\log(\triangle w)}
\end{equation}

The length of the windowed segment along with the size of the window offset used can both affect the resulting VFDT. The best window length and window offset will be unique and specific for any given type of signal. For the RF signals analyzed in this paper, the main factors that resulted in needing to vary the window size and offset seemed to be the sample rate of the base signal along with the stationarity of the signal. Generally, the best window length and window offset are subjective and commonly determined through experimentation. It can be useful to have the window offset size be smaller than the window length as this causes overlap in adjacent windows and typically yields better results. Also note that the smaller the window length and window offset are, the larger the resulting VFDT will be in terms of analyzed segments. 



%Here is how to add a table (Table~\ref{table:lora}).

%\begin{table}
%\centering
%\small
%\begin{tabular}{|c|c|c|c|c|c|}
%    \hline
%    \textbf{Config.} & \begin{tabular}{@{}c@{}}\textbf{Spreading} \\ \textbf{Factor}\end{tabular} & \textbf{BW} & \begin{tabular}{@{}c@{}}\textbf{Tx} \\ \textbf{Power}\end{tabular} &  \begin{tabular}{@{}c@{}}\textbf{Coding} \\ \textbf{Rate}\end{tabular}&\textbf{Bit Rate}\\
%    \hline
%    1 & 7 & 125kHz & 20dBm & 4/5 & 5470bps \\
%    2 & 8 & 125kHz & 20dBm & 4/5 & 3125bps \\
%    3 & 11 & 125kHz & 20dBm & 4/5 & 537bps \\
%    4 & 12 & 125kHz & 20dBm & 4/5 & 293bps \\
%    \hline  
%\end{tabular}
%\caption{Different LoRa transmitter configurations.}
%\label{table:lora}
%\end{table}
